Risk-Aware Linear Bandits: Theory and Applications in Smart Order Routing

Motivated by practical considerations in machine learning for financial decision-making, such as risk aversion and large action space, we consider risk-aware bandits optimization with applications in smart order routing (SOR). Specifically, based on preliminary observations of linear price impacts made from the NASDAQ ITCH dataset, we initiate the study of risk-aware linear bandits. In this setting, we aim at minimizing regret, which measures our performance deficit compared to the optimum's, under the mean-variance metric when facing a set of actions whose rewards are linear functions of (initially) unknown parameters. Driven by the variance-minimizing globally-optimal (G-optimal) design, we propose the novel instance-independent Risk-Aware Explore-then-Commit (RISE) algorithm and the instance-dependent Risk-Aware Successive Elimination (RISE++) algorithm. Then, we rigorously analyze their near-optimal regret upper bounds to show that, by leveraging the linear structure, our algorithms can dramatically reduce the regret when compared to existing methods. Finally, we demonstrate the performance of the algorithms by conducting extensive numerical experiments in the SOR setup using both synthetic datasets and the NASDAQ ITCH dataset. Our results reveal that 1) The linear structure assumption can indeed be well supported by the Nasdaq dataset; and more importantly 2) Both RISE and RISE++ can significantly outperform the competing methods, in terms of regret, especially in complex decision-making scenarios.

==> time_machine/backup/backup_numerical_Dec_2022.tex <==

\section{Application: Smart Order Routing}
\label{sec:numerical}

In this section, we apply {\rise } algorithm and \risepp~ algorithm to the SOR problem,
%In order to execute a trade of a given asset, 
in which market participants  have the opportunity to split the trade and submit orders to different venues, including both lit pools and dark pools. This  could potentially improve the overall execution price and quantity. Both the decision and the outcome are influenced by the characteristics of different venues as well as the structure of transaction fees and rebates across different venues.

\noindent{\bf Dark Pools:} Dark pools are private exchanges for trading securities that are not accessible by the investing public. Also known as ``dark pools of liquidity,'' the name of these exchanges is a reference to their complete lack of transparency. Dark pools were created in order to facilitate block trading by institutional investors who did not wish to impact the markets with their large orders and obtain adverse prices for their trades.

\noindent{\bf Lit Pools and Limit Order Books:} Unlike dark pools, where prices at which participants are willing to trade are not revealed, lit pools do display bid offers and ask offers in different assets. Primary exchanges operate in such a way that available liquidity is displayed at all times and form the bulk of the lit pools available to traders through the so-called  Limit Order Books (LOB). An LOB is a list of orders that a trading venue, for example the NASDAQ exchange, uses to record the interest of buyers and sellers in a particular financial asset. There are two types of orders the buyers (sellers) can submit: a \emph{limit buy (sell) order} with a preferred price for a given volume of the asset or a \emph{market buy (sell) order} with a given volume which will be immediately executed with the best available limit sell (buy) orders. 
Therefore, limit orders have a price guarantee but are not guaranteed to be executed, whereas market orders are executed immediately at the best available price. The lowest price of all  limit sell orders is called the \emph{ask} price, and the highest price of all limit buy orders is called the \emph{bid} price. The difference between the ask and bid is known as the \emph{spread} and the average of the ask and bid is known as the \emph{mid-price}. 
    
A matching engine uses the LOB to store pending orders and match them with the incoming buy and sell orders. This typically follows the price-time priority rule \cite{preis2011price}, whereby orders are first ranked according to their price. Multiple orders having the same price are then ranked according to the time they were entered.

For the SOR problem, the most important characteristics of different dark pools are the chances of being  matched with a counter party and the price (dis)advantages whereas the relevant characteristics of lit pools include the order flows, queue sizes, and cancellation rates. These characteristics are often not available (initially) and could be learned by trial and error.

\subsection{Setup for Numerical Experiment}
Consider a trader who faces a task to sell certain shares of a given  asset in a repeated setting. The trader has access to $(J+N)$ venues where  $J$ of them are lit pools and  $N$ of them are  dark pools. 

In each iteration $t$, the trader receives a task to sell $S_t$ shares of the given asset where $S_t$ are sampled iid from some unknown distribution $\mu_S$.  Assume that $\mu_S$ is defined on a compact set  such that $s \leq S_t \leq S$ holds $\mu_S$-almost surely with some $0<s<S$.

Denote $A_t = (L_t^1,\cdots,L_t^J,V_t^1,\cdots,V_t^N,M_t)\in\mathbb{R}^{J+N+1}$ as the allocation taken by the trader at time $t$, where $L_t^j$ is the quantity of limit sell orders submitted to the $j$th lit pool to join the queue of the best ask price level $(1\leq j \leq J)$, $V^{n}_t$ is the quantity submitted  to the $n$th dark pool, and $M_t$ is the amount of market orders sent to the lit pools which will be executed  at the highest best bid prices  plus a small fee. We assume that $\sum_{j=1}^J L_t^j + \sum_{n=1}^N V_t^n +M_t = S_t$.

\drg{@ Prof. Xu: Do we have any reference to the following stylized fact? }

The reward is assumed to follow:
\begin{eqnarray}
%X_t &=& \sum_{n=1}^N\Big(p^{d,n} V_t^n + \varepsilon^{d,n}(V_t^n) \Big)\nonumber\\&&+ \sum_{j=1}^J\Big(p^{l,j} L_t^j + \varepsilon^{l,j}_t(L_t^j)\Big) + {p}^m M_t + \varepsilon^{m}_t(M_t),
X_t &=& \sum_{n=1}^N\,p^{d,n} V_t^n  + \sum_{j=1}^J \, p^{l,j} L_t^j  + {p}^m M_t  + \eta_t(A_t),
\end{eqnarray}
where $p^m$ is the average trading price of market orders, $p^{d,n}$ is the average trading price of the orders at the $n$th \underline{d}ark pool, and $p^{l,j}$ is the average trading price of the \underline{l}imit sell orders sent to the $j$th lit pool. We assume that
\begin{equation} \label{eq:ceofficients_constraints_1}
p^m < \min_{1\leq n \leq N}\{p^{d,n}\} \leq \max_{1\leq n \leq N}\{p^{d,n}\} < \min_{1\leq j \leq J}\{p^{l,j}\}.
\end{equation}
This is based on the following facts:
\begin{itemize}
    \item The executed limit orders (in lit pools) have the best price privilege compared to market orders and executed dark pool orders.
    \item Most of the executed dark pool orders can be traded at the mid-price of the lit pools, which is better than the price of the market orders (with a margin of half bid-ask spread).
    \item Both limit orders and dark pool orders are not guaranteed for execution. Non-executed quantities will be sent as market orders for immediate execution at the end of each iteration.
\end{itemize}

The noise term  in the reward follows $\eta_t(A_t)\sim \mathcal{N}(0,f(A_t))$ with
\begin{eqnarray}
f(A_t) = \sum_{n=1}^N (\sigma^{d,n})^2 V_t^n +\sum_{j=1}^J (\sigma^{l,j})^2 L_t^j +(\sigma^m)^2 M_t + \omega.
\end{eqnarray}
%$\varepsilon_t^{d,n}(V)\sim \mathcal{N}(0,(\sigma^{d,n})^2 V + \omega)$, $\varepsilon_t^{l,j}(L)\sim \mathcal{N}(0,(\sigma^{l,j})^2 L + \omega)$, and $\varepsilon_t^{m}(M)\sim \mathcal{N}(0,(\sigma^{m})^2 M + \omega)$. 
Here we assume that 
\begin{equation} \label{eq:ceofficients_constraints_2}
    0<\sigma^{m} < \sigma^{d,n}< \sigma^{l,j},
\end{equation}
for all $1 \leq n \leq N$ and $1 \leq j \leq J$. This assumption is based on the following characteristics of different venues:
\begin{itemize}
    \item Uncertainty is (more or less) proportional to the trading quantity. Hence we assume the variance is linear in the trading quantity.
    \item Limit orders have the largest execution uncertainties whereas market orders have the least execution uncertainties.
\end{itemize}


\iffalse
That is, the limit orders with quantities $(L_t^1,\cdots, L_t^K)$ join queues of $(Q_t^{a,1},\cdots, Q_t^{a,K})$ orders in $K$ limit sell order books, where $Q_t^{a,k} \ge 0$ $(1\leq k \leq K)$.  Then the filled amounts at the end of iteration $t$ can be written as a function of their initial queue position and future order flow \cite{cont2017optimal}:
\begin{eqnarray}\label{eq:firfull_amnt}
\min(\max(\xi_t^k - Q_t^{a,k}, 0), L_t^k) = (\xi_t^k-Q_t^{a,k})_+ - (\xi_t^k - Q_t^{a,k} - L_t^k)_+,
\end{eqnarray}
where the notation $(x)_+ = \max(0,x)$. Here $\xi_t^k:=D_t^k+E_t^k$ is the total outflow from the front of the $k$-th queue which consists of
order cancellations $E_t^k$ that occurred before the end of iteration $t$ from queue positions in front of our trader's order and marketable orders $D_t^k$ that reach the $k$-th exchange before the end of iteration $t$.  Note that the fulfilled amounts are random because they depend on queue outflows $\xi_t=(\xi_t^1,\cdots,\xi_t^K)$ the $t$-th iteration which are modeled as random variables with an unknown distribution $\mu_{\xi}$. The instantaneous queue outflows $\xi_t$ can be observed at the end of iteration $t$.


Dark pools are type of markets that are designed to facilitate large transactions. A
key aspect of dark pools is the {\it censored feedback} that
the trader receives. When a
certain number of shares  $V^{n}_t$ is allocated to dark pool $n$,  this dark pool $n$ trades as many
of the allocated shares $V_t^n$ with the available
liquidity $U_t^n$ \cite{agarwal2010optimal}. The trader only finds out how many of these
allocated shares were successfully traded at each dark
pool (i.e., $\min(U_t^n,V_t^n)$), but not how many would have been traded if
more were allocated (i.e., $U_t^i$) at price level $P_t^n$. Both  the price level $P_t^n$ and the executed quantity  $\min(U_t^n,V_t^n)$ will be revealed at the end of the iteration $t$.


Denote $M_t$ as the amount of market orders sent to the LOB which will be executed at the lit pool with the biggest best bid price $\max_{1\leq k \leq K}P^{b,k}_{t}$ plus a small fee. For quantities sent to the lit pools as limit orders and to dark pools that are not successfully executed, they will be routed to lit pools as market orders to seek for immediate execution. 

To summarize, the execution reward of the allocation $X_t = (M_t, L_t^1,.. ., L_t^K,V_t^1,\cdots,V_t^K)$ across dark pools and lit pools is defined as:
\begin{eqnarray}\label{eq:reward}
&&R_t(X_t) := \\
&&\underbrace{\sum_{n=1}^N P^n_t \min\{V_t^n,U_t^n\}}_{\mbox{reward from successful dark pool orders}}\nonumber \\
&&+\underbrace{\sum_{k=1}^K (P_t^{a,k} + r_k)((\xi_t^k - Q_t^{a,k})_+ - (\xi_t^k - Q_t^{a,k} - L_t^k)_+)}_{\mbox{reward from successful limit orders}}\nonumber\\
&&+\underbrace{\Big( M_t + \sum_{n=1}^N (V_t^n-U_t^n)_+ + (L_t^k - \xi_t^k + Q_t^{a,k})_+ \Big) \left(\max_{1\leq k \leq K}P^{b,k}_{t}+f\right)}_{\mbox{ reward from market orders}},\nonumber
\end{eqnarray}
where $f>0$ is a fee for market orders and $r_k>0$ are effective
rebates for limit orders on exchanges $k = 1,\cdots,K$. These quantities are known before the allocation $X_t$ has been made.

\subsection{Linear Approximation of the Reward} \label{sec:linear_approximation} Key observation is that market orders have the least preferable execution price and the smallest execution uncertainty. Limit orders have the best execution price but also the largest uncertainty of being executed (against the market buy orders), especially when the volume of the order is large. 

Most of the dark pool orders can be executed at the average mid-price across all lit pools but they have different uncertainties in terms of the quantities to be executed. Recall that the quantities that are not executed in the $n$th dark pool, $(V_t^n-U_t^n)_+$, will be submitted as market orders to the lit pools for immediate execution. This leads to different {\it average execution price} and different uncertainties of the reward from each dark pool.
\eqref{eq:reward} can be approximated by the following linear reward:
\begin{eqnarray}
\tilde{R}_t(X_t) &=& \sum_{n=1}^N\Big(p^{d,n} V_t^n + 
\varepsilon^{d,n}(V_t^n) \Big)\nonumber\\
&&+ \sum_{k=1}^K\Big(p^{l,k} L_t^k + \varepsilon^{l,k}_t(L_t^k)\Big) + p^m M_t + \varepsilon^{m}_t(M_t),
\end{eqnarray}
where $p^m$ is the average trading price of market orders, $p^{d,n}$ is the average trading price of the orders at the $n$th dark pool, and $p^{l,k}$ is the average trading price of the limit sell orders sent to the $k$th lit pool. We assume that
$p^m < \min_{1\leq n \leq N}\{p^{d,n}\} \leq \max_{1\leq n \leq N}\{p^{d,n}\} < \min_{1\leq k \leq K}\{p^{l,k}\}$. Here $\varepsilon_t^{d,n}(V)\sim \mathcal{N}(0,(\sigma^{d,n})^2 V + \delta)$, $\varepsilon_t^{l,k}(L)\sim \mathcal{N}(0,(\sigma^{l,k})^2 L + \delta)$, and $\varepsilon_t^{m}(M)\sim \mathcal{N}(0,(\sigma^{m})^2 M + \delta)$ with $0<\sigma^{m} < \sigma^{d,n}< \sigma^{l,k}$ for all $1 \leq n \leq N$ and $1 \leq k \leq K$.

\fi


\subsection{Numerical Results}

In this section, we briefly showcase the superiority of \rise~ and \risepp~ for the SOR problem using synthetic data. 

\noindent{\bf Choice of Parameters:} For simplicity, we assume that the number of shares the trader needs to sell in each iteration is fixed, i.e. $S_t=S$ over time. Also, we consider only non-negative integer allocations of $S$ orders into $d = J + N + 1$ venues. 
%\Ruihao{It appears that there are two setups here, one in the title of Section 4.1 and one in the above paragraph, can we somehow merge them?}

Throughout the experiments, we set $\rho=2$ and vary values of $d$ and $S$. We set $\omega=1$ and scale the action vectors accordingly so that the norm of actions is less than 1. 
The model coefficients are randomly generated such that \eqref{eq:ceofficients_constraints_1} and \eqref{eq:ceofficients_constraints_2} are satisfied. See Table~\ref{tab:1} for the model coefficients we used for three different scenarios.
%\Jingwei{table updated}
\begin{footnotesize}
\begin{table}[htbp]
  \centering
  \caption{Model parameters used for experiments}
    \begin{tabular}{ccccccc}
    \toprule
    \multicolumn{7}{c}{Scenario I ($d=4$)} \\
    \midrule
    $p$ & 0.1316 & 0.3218 & 0.5800 & 0.7367 &    &  \\
    $\sigma^2$ & 0.2506 & 0.2902 & 0.5090 & 0.7706 &    &  \\
    \midrule
    \multicolumn{7}{c}{Scenario II ($d=5$)} \\
    \midrule
    $p$ & 0.1121 & 0.2742 & 0.4942 & 0.5232 & 0.6278 &  \\
    $\sigma^2$ & 0.2318 & 0.2685 & 0.3798 & 0.4709 & 0.7129 &  \\
    \midrule
    \multicolumn{7}{c}{Scenario III ($d=6$)} \\
    \midrule
    $p$ & 0.1081 & 0.2641 & 0.2645 & 0.4767 & 0.5047 & 0.6055 \\
    $\sigma^2$ & 0.1631 & 0.1889 & 0.2672 & 0.3313 & 0.5015 & 0.7106 \\
    \end{tabular}%
  \label{tab:1}%
\end{table}%
\end{footnotesize}

\noindent{\bf Implementation details:} We note that when implementing \rise, rather than strictly follow \eqref{eq:n_a} and \eqref{eq:n} to decide the length of exploration phase,  we set $n = \lceil d T^{2/3} \rceil$ in the experiments for practical convenience.
Also, when implementing \risepp,  we set $n_{\ell, a} = \left\lceil 0.0001 \cdot \frac{d^{3}  \log(d) Q_{\ell}^{*} (a) }{\varepsilon_{\ell}^{2}} \log^2 \left( K T^2  \right)\right\rceil$ rather than strictly follow \eqref{eq:phase_elimination_phase_length}.
Moreover,    we regularize the design matrix as $ V_{(\ell)}=\sum_{a \in \mathcal{A}_{\ell}} n_{\ell,a}  a a^{\top} + I_d $ to avoid singularity issue for \risepp. % rather than using $ V_{(\ell)}=\sum_{a \in \mathcal{A}_{\ell}} n_{\ell,a}  a a^{\top}$ ,


\noindent{\bf Criterion and Benchmark Algorithms:} In view of the connection between proxy regret and intermediate regret established in proposition~\ref{prop:regret_trans}, we use the intermediate regret as a performance measure of different algorithms. 

We compare \rise~ and \risepp~ with two algorithms proposed by \cite{sani2012risk} for the MAB problem. 
The first one is a variation of the UCB policy (referred to as UCB(MAB)) and the second a variation of the exploration-and-exploitation policy (referred to as ExpExp(MAB)).  To apply these two algorithms to the SOR problem, we simply let all non-negative integer allocations of $S$ orders into $d$ venues be the whole action space.  The implementations of the UCB(MAB) and ExpExp(MAB) strictly follow the descriptions in  \cite{sani2012risk}. 


\begin{figure}[!ht]
	\centering
	\subfigure[$d=4, S=4, K=35$ (Scenario I).]{\includegraphics[width=8cm,height=5.5cm]{plots/d=4,S=4.png} \label{fig:1_d4S4} }
	\subfigure[$d=5, S=4, K=70$ (Scenario II).]{\includegraphics[width=8cm,height=5.5cm]{plots/d=5,S=4.png} \label{fig:2_d5S4}	}
	\subfigure[$d=6, S=4, K = 126$ (Scenario III).]{\includegraphics[width=8cm,height=5.5cm]{plots/d=6,S=4.png} \label{fig:3_d6S4}	}
	\subfigure[$d=6, S=8, K=1287$ (Scenario III).]{\includegraphics[width=8cm,height=5.5cm]{plots/d=6,S=8.png} \label{fig:4_d6S8}	}
	\caption{Intermediate regrets of different algorithms over $T$.}
	\label{fig:intermediate_regret}
\end{figure}


\noindent{\bf Numerical Performance and Discussion:} 
We provide one plot for scenario I (cf. Figure \ref{fig:1_d4S4}), one plot for scenario II (cf. Figure \ref{fig:2_d5S4}), and two plots for scenario III with different $S$ values (cf. Figures \ref{fig:3_d6S4}- \ref{fig:4_d6S8}).
First of all, it is evident that \rise~and \risepp~ have the best empirical performances in all three different scenarios. 
Next, we observe in Figure~\ref{fig:1_d4S4} and \ref{fig:2_d5S4} that when action space is relatively small ($K=35$ or $K=70$), the UCB(MAB) still exhibits a logarithmic regret growth rate. 
It may outperform other three algorithms eventually, but its performance is the worst in the time frame we considered.
% However, as the action space grows, in Figure~\ref{fig:2} ($K=70$), though the UCB(MAB)   
% The empirical findings are consistent with the theoretical results. 
%Recall that instance-dependent intermediate regret growth rate of UCB(MAB) is $O(K)$ (with log dependence in $T$) and the instance-independent intermediate regret growth rate of ExpExp(MAB) is $O(K T^{2/3})$. This reemphasizes that linear bandit is more sample efficient when the action space is large.

Furthermore, through Figure~\ref{fig:1_d4S4} to \ref{fig:4_d6S8}, the performances of both UCB(MAB) and ExpExp(MAB) get worse as $K$ grows. 
Figure~\ref{fig:4_d6S8}  shows that regrets of them grow linearly when the action space is large ($K=1287$). 
Specifically, since the length of its exploration phase is $K (T/14)^{2/3}$,   UCB(ExpExp) will  uniformly explore over the whole horizon when $K$ is large.  
{On the contrary, \rise~and~\risepp~ are able to fully utilize the linear structure of the problem and their regret growth rates do not rely on $K$, the size of action space. 
Therefore, \rise~and \risepp~ are especially competent for tasks with a huge action space. 
However, the performance comparison between \rise~and \risepp~ is more complex, which may depend on specific instances. 
}
\iffalse
\begin{figure}[htbp] 
  \begin{minipage}{\linewidth}
    \makebox[.5\linewidth]{\includegraphics[width=.45\linewidth]{plots/d=4,S=4.png}}%
    \makebox[.5\linewidth]{\includegraphics[width=.45\linewidth]{plots/d=5,S=4.png}}

    \makebox[.5\linewidth]{\small (a) $d=4, S=4, K=35$ (Scenario I).}%
    \makebox[.5\linewidth]{\small (b) $d=5, S=4, K=70$ (Scenario II).}%

    \medskip

    \makebox[.5\linewidth]{\includegraphics[width=.45\linewidth]{plots/d=6,S=4.png}}%
    \makebox[.5\linewidth]{\includegraphics[width=.45\linewidth]{plots/d=6,S=8.png}}

    \makebox[.5\linewidth]{\small (c) $d=6, S=4, K = 126$ (Scenario III).}%
    \makebox[.5\linewidth]{\small (d) $d=6, S=8, K=1287$ (Scenario III).}%
  \end{minipage}%
  \caption{Intermediate regrets of different algorithms over $T$.}
  \label{fig:numerical_regret}
\end{figure}
\fi 

\iffalse
\Ruihao{ 2 by 2 }
\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.6\linewidth]{plots/d=4,S=4.png}
  \caption{$d=4, S=4, K=35$ (Scenario I).}
  \label{fig:1_d4S4}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.6\linewidth]{plots/d=5,S=4.png}
  \caption{$d=5, S=4, K=70$ (Scenario II).}
  \label{fig:2_d5S4}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.6\linewidth]{plots/d=6,S=4.png}
  \caption{$d=6, S=4, K = 126$ (Scenario III).}
  \label{fig:3_d6S4}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.6\linewidth]{plots/d=6,S=8.png}
  \caption{$d=6, S=8, K=1287$ (Scenario III).}
  \label{fig:4_d6S8}
\end{figure}
\fi 

\subsection{}



==> time_machine/backup/numerical.tex <==

\section{Application: Smart Order Routing}
\label{sec:numerical}

In this section, we apply {\rise } algorithm and \risepp~algorithm to the smart order routing (SOR) problem.
In what follows, we first explain the problem in depth and model it in the framework of linear bandits. 
Then, we test our algorithms on both a synthetic dataset and the NASDAQ ITCH dataset. 

%In order to execute a trade of a given asset, 
Usually, the SOR problem arises for big institutions who need to liquidate a large amount of stocks. 
To do so, they can % in which market participants have the opportunity to
split the trade and submit orders to different venues, including both lit pools and dark pools. 
This could potentially improve the overall execution price and minimize the total market impact. 
Both the decision and the outcome are influenced by the characteristics of different venues as well as the structure of transaction fees and rebates across different venues.
Interested readers are referred to for instance, \cite{JP_SOR}, for further information.

\noindent{\bf Dark Pools:} % Dark pools are private exchanges for trading securities that are not accessible by the investing public. Also known as ``dark pools of liquidity'', the name of these exchanges is a reference to their lack of transparency. Dark pools were created in order to facilitate block trading by institutional investors who did not wish to impact the markets with their large orders and obtain adverse prices for their trades.
Dark pools are private exchanges for trading securities that are not accessible by the investing public.  These exchanges, referred to as ``dark pools of liquidity'' due to their lack of transparency, were established to allow institutional investors to trade large amounts of securities without triggering too much impact on the market and facing adverse prices for their trades.


\noindent{\bf Lit Pools and Limit Order Books:} Unlike dark pools, where prices at which participants are willing to trade are not revealed, lit pools do display bid offers and ask offers for different assets. Primary exchanges operate in such a way that available liquidity is displayed at all times.
They form the bulk of the lit pools available to traders through the so-called  Limit Order Books (LOB). An LOB is a list of orders that a trading venue (\eg, the NASDAQ exchange) uses to record the interest of buyers and sellers in a particular financial asset. There are two types of orders the buyers (sellers) can submit: a \emph{limit buy (sell) order} with a preferred price for a given volume of the asset or a \emph{market buy (sell) order} with a given volume which will be immediately executed with the best available limit sell (buy) orders. 
Therefore, limit orders have a price guarantee but are not guaranteed to be executed, whereas market orders are executed immediately at the best available price. The lowest price of all  limit sell orders is called the \emph{best ask} price, and the highest price of all limit buy orders is called the \emph{best bid} price. The difference between the best ask and best bid is known as the \emph{spread} and the average of the best ask and best bid is known as the \emph{mid-price}. 
    
A matching engine uses the LOB to store pending orders and match them with incoming buy and sell orders. This typically follows the price-time priority rule \citep{preis2011price}, whereby orders are first ranked according to their price. Multiple orders having the same price are then ranked according to the time they were entered.
According to \cite{rosenblatt_report}, dark pools executed approximately 15.03\% of US equity volume in December 2022. 


For the SOR problem, the most important characteristics of different dark pools are the chances of being  matched with a counterparty and the price (dis)advantages; whereas the relevant characteristics of lit pools include the order flows, queue sizes, and cancellation rates. These characteristics are often not available (initially) and could be learned by trial and error.

\subsection{Modeling SOR in the Framework of Linear Bandits}
Consider a trader who faces a task of selling certain shares of a given  asset in a repeated setting. The trader has access to $(J+N)$ venues where $J$ of them are lit pools and  $N$ of them are  dark pools. 

In each iteration $t$, the trader receives a task to sell $S$ shares of the given asset where $S$ is a known constant.
In the context of SOR problem, we overload $A_t$ to be $A_t = (M_t^1,\cdots,M_t^J, L_t^1,\cdots,L_t^J, D_t^1,\cdots,D_t^N )\in\mathbb{R}^{J+J+N}$ as the allocation taken by the trader at time $t$, where $M_t^j$ is the number of market orders submitted to the $j$th lit pool which will be executed against the limit buy orders, 
$L_t^j$ is the number of limit sell orders submitted to the $j$th lit pool to join the queue of the best ask price level, 
and $D_t^n$ is the quantity submitted to the $n$th dark pool. 
In view of the linear bandit framework, the dimension of the actions is the number of venues, \ie, $d = J + J + N$. 
For $A_t$ to be admissible, we require that $ \sum_{j=1}^{J} M_t^j + \sum_{j=1}^{J} L_t^j  + \sum_{n=1}^{N} D_t^n = S$.

% Assume that $\mu_S$ is defined on a compact set  such that $s \leq S_t \leq S$ holds $\mu_S$-almost surely with some $0<s<S$. Denote $A_t = (L_t^1,\cdots,L_t^J,V_t^1,\cdots,V_t^N,M_t)\in\mathbb{R}^{J+N+1}$ as the allocation taken by the trader at time $t$, where $L_t^j$ is the quantity of limit sell orders submitted to the $j$th lit pool to join the queue of the best ask price level $(1\leq j \leq J)$, $V^{n}_t$ is the quantity submitted  to the $n$th dark pool, and $M_t$ is the amount of market orders sent to the lit pools which will be executed  at the highest best bid prices  plus a small fee. We assume that $\sum_{j=1}^J L_t^j + \sum_{n=1}^N V_t^n +M_t = S_t$.
\Jingwei{To include quadratic terms }
The reward is assumed to have a linear form in $A_t$:
\begin{eqnarray}
%X_t &=& \sum_{n=1}^N\Big(p^{d,n} V_t^n + \varepsilon^{d,n}(V_t^n) \Big)\nonumber\\&&+ \sum_{j=1}^J\Big(p^{l,j} L_t^j + \varepsilon^{l,j}_t(L_t^j)\Big) + {p}^m M_t + \varepsilon^{m}_t(M_t),
% X_t &=& \sum_{n=1}^N\,p^{d,n} V_t^n  + \sum_{j=1}^J \, p^{l,j} L_t^j  + {p}^m M_t  + \eta_t(A_t),
X_t &=&  
\sum_{j=1}^J \, p^{\texttt{m},j} M_t^j 
+ \sum_{j=1}^J \, p^{\texttt{l},j} L_t^j 
+ \sum_{n=1}^N \, p^{\texttt{d},n} D_t^n    
+ \eta_t(A_t), \label{eq:sor_mean_model}
\end{eqnarray}
where $ p^{\texttt{m},\cdot } , p^{\texttt{l},\cdot}, p^{\texttt{d},\cdot}$ are the average {\it unit profit and loss (PnL)} of the \underline{m}arket order, \underline{l}imit order and \underline{d}ark pool respectively.
The unit PnL is defined to be the trading price subtracted by the prevailing mid-price of the stock. % under the market condition. 
% \renyuan{This is called profit and loos (PnL) in the literature. Standardized trading price is a bit misleading.}
We note that PnL can be both positive and negative. 

In view of Eq.~\eqref{eq:var_def}, we assume that the noise term in the reward follows $\eta_t(A_t)\sim \mathcal{N}(0,f(A_t))$ with
\begin{equation} 
f(A_t) = \sum_{j=1}^J \, (\sigma^{\texttt{m},j})^2 M_t^j 
+ \sum_{j=1}^J \, (\sigma^{\texttt{l},j})^2 L_t^j 
+ \sum_{n=1}^N \, (\sigma^{\texttt{d},n})^2 D_t^n 
+ \omega, \label{eq:sor_var_model}
\end{equation}
where $\omega>0$ is a positive constant to guarantee that the variance is well-defined.  Since uncertainty is (more or less) proportional to the trading quantity,  we assume the variance is linear in the trading quantity.

Note that the linear assumptions in \eqref{eq:sor_mean_model} and \eqref{eq:sor_var_model} are consistent with the empirical observations from real data. See Figure \ref{fig:tsla} for the details.

\iffalse
That is, the limit orders with quantities $(L_t^1,\cdots, L_t^K)$ join queues of $(Q_t^{a,1},\cdots, Q_t^{a,K})$ orders in $K$ limit sell order books, where $Q_t^{a,k} \ge 0$ $(1\leq k \leq K)$.  Then the filled amounts at the end of iteration $t$ can be written as a function of their initial queue position and future order flow \cite{cont2017optimal}:
\begin{eqnarray}\label{eq:firfull_amnt}
\min(\max(\xi_t^k - Q_t^{a,k}, 0), L_t^k) = (\xi_t^k-Q_t^{a,k})_+ - (\xi_t^k - Q_t^{a,k} - L_t^k)_+,
\end{eqnarray}
where the notation $(x)_+ = \max(0,x)$. Here $\xi_t^k:=D_t^k+E_t^k$ is the total outflow from the front of the $k$-th queue which consists of
order cancellations $E_t^k$ that occurred before the end of iteration $t$ from queue positions in front of our trader's order and marketable orders $D_t^k$ that reach the $k$-th exchange before the end of iteration $t$.  Note that the fulfilled amounts are random because they depend on queue outflows $\xi_t=(\xi_t^1,\cdots,\xi_t^K)$ the $t$-th iteration which are modeled as random variables with an unknown distribution $\mu_{\xi}$. The instantaneous queue outflows $\xi_t$ can be observed at the end of iteration $t$.

Dark pools are type of markets that are designed to facilitate large transactions. A key aspect of dark pools is the {\it censored feedback} that
the trader receives. When a certain number of shares  $V^{n}_t$ is allocated to dark pool $n$,  this dark pool $n$ trades as many
of the allocated shares $V_t^n$ with the available
liquidity $U_t^n$ \cite{agarwal2010optimal}. 
The trader only finds out how many of these allocated shares were successfully traded at each dark
pool (\textit{i.e.}, $\min(U_t^n,V_t^n)$), but not how many would have been traded if more were allocated (\textit{i.e.}, $U_t^i$) at price level $P_t^n$. Both  the price level $P_t^n$ and the executed quantity  $\min(U_t^n,V_t^n)$ will be revealed at the end of the iteration $t$.


Denote $M_t$ as the amount of market orders sent to the LOB which will be executed at the lit pool with the biggest best bid price $\max_{1\leq k \leq K}P^{b,k}_{t}$ plus a small fee. For quantities sent to the lit pools as limit orders and to dark pools that are not successfully executed, they will be routed to lit pools as market orders to seek for immediate execution. 

To summarize, the execution reward of the allocation $X_t = (M_t, L_t^1,.. ., L_t^K,V_t^1,\cdots,V_t^K)$ across dark pools and lit pools is defined as:
\begin{eqnarray}\label{eq:reward}
&&R_t(X_t) := \\
&&\underbrace{\sum_{n=1}^N P^n_t \min\{V_t^n,U_t^n\}}_{\mbox{reward from successful dark pool orders}}\nonumber \\
&&+\underbrace{\sum_{k=1}^K (P_t^{a,k} + r_k)((\xi_t^k - Q_t^{a,k})_+ - (\xi_t^k - Q_t^{a,k} - L_t^k)_+)}_{\mbox{reward from successful limit orders}}\nonumber\\
&&+\underbrace{\Big( M_t + \sum_{n=1}^N (V_t^n-U_t^n)_+ + (L_t^k - \xi_t^k + Q_t^{a,k})_+ \Big) \left(\max_{1\leq k \leq K}P^{b,k}_{t}+f\right)}_{\mbox{ reward from market orders}},\nonumber
\end{eqnarray}
where $f>0$ is a fee for market orders and $r_k>0$ are effective
rebates for limit orders on exchanges $k = 1,\cdots,K$. These quantities are known before the allocation $X_t$ has been made.

\subsection{Linear Approximation of the Reward} \label{sec:linear_approximation} Key observation is that market orders have the least preferable execution price and the smallest execution uncertainty. Limit orders have the best execution price but also the largest uncertainty of being executed (against the market buy orders), especially when the volume of the order is large. 

Most of the dark pool orders can be executed at the average mid-price across all lit pools but they have different uncertainties in terms of the quantities to be executed. Recall that the quantities that are not executed in the $n$th dark pool, $(V_t^n-U_t^n)_+$, will be submitted as market orders to the lit pools for immediate execution. This leads to different {\it average execution price} and different uncertainties of the reward from each dark pool.
\eqref{eq:reward} can be approximated by the following linear reward:
\begin{eqnarray}
\tilde{R}_t(X_t) &=& \sum_{n=1}^N\Big(p^{d,n} V_t^n + 
\varepsilon^{d,n}(V_t^n) \Big)\nonumber\\
&&+ \sum_{k=1}^K\Big(p^{l,k} L_t^k + \varepsilon^{l,k}_t(L_t^k)\Big) + p^m M_t + \varepsilon^{m}_t(M_t),
\end{eqnarray}
where $p^m$ is the average trading price of market orders, $p^{d,n}$ is the average trading price of the orders at the $n$th dark pool, and $p^{l,k}$ is the average trading price of the limit sell orders sent to the $k$th lit pool. We assume that
$p^m < \min_{1\leq n \leq N}\{p^{d,n}\} \leq \max_{1\leq n \leq N}\{p^{d,n}\} < \min_{1\leq k \leq K}\{p^{l,k}\}$. Here $\varepsilon_t^{d,n}(V)\sim \mathcal{N}(0,(\sigma^{d,n})^2 V + \delta)$, $\varepsilon_t^{l,k}(L)\sim \mathcal{N}(0,(\sigma^{l,k})^2 L + \delta)$, and $\varepsilon_t^{m}(M)\sim \mathcal{N}(0,(\sigma^{m})^2 M + \delta)$ with $0<\sigma^{m} < \sigma^{d,n}< \sigma^{l,k}$ for all $1 \leq n \leq N$ and $1 \leq k \leq K$.

\fi


\subsection{A Synthetic Example}

In this section, we first briefly showcase the superiority of \rise~and \risepp~solving the SOR problem using synthetic data. 

\noindent{\bf Choice of Parameters:} For simplicity, we consider only non-negative integer allocations of $S$ orders into $d$ venues. 
% \renyuan{Why you use $d$ here? It is not consistent with previous section. Also, $d$ is used for something else, see Eqn 31...}
% \Jingwei{In our model, $d$ is the dimension of each action vector. Each element in such a vector represents the number of stocks submitted to the corresponding venue. In Eq. 31, I used an un-italicized d.  } \renyuan{Please mention $d=J+J+N$ in the previous section (to connect the notation with Section 2) otherwise it is a bit misleading.}
Throughout the experiments, we set the risk-aversion parameter $\rho=2$  and vary the choices of $d$ and $S$. We set $\omega=1$ and scale the action vectors accordingly so that the norms of actions are less than one. 
To make the scenario interesting and non-trivial, the model coefficients are set to satisfy the following assumptions:
\begin{eqnarray} 
  & p^{\texttt{m},\cdot } < p^{\texttt{d},\cdot} < p^{\texttt{l},\cdot},\label{eq:ceofficients_constraints_1} \\
 &   0<\sigma^{\texttt{m},\cdot } < \sigma^{\texttt{d},\cdot} < \sigma^{\texttt{l},\cdot}.\label{eq:ceofficients_constraints_2}
\end{eqnarray}
Assumption \eqref{eq:ceofficients_constraints_1}  is made based on the following stylist facts:
\begin{itemize}
    \item Executed limit orders in lit pools have a price advantage over both market orders and executed dark pool orders. % The executed limit orders (in lit pools) have the best price privilege compared to market orders and executed dark pool orders.
    \item Most orders at competitive or major dark pools can be traded at the mid-price of lit pools, providing a better price than market orders with a margin of half the bid-ask spread. % For competitive or major dark pool venues, most of the  orders can be traded at the mid-price of the lit pools, which is better than the price of the market orders (with a margin of half bid-ask spread).
    \item Neither limit nor dark pool orders are guaranteed to be executed. Any unfulfilled quantities will be sent as market orders for immediate execution at the end of each iteration.
\end{itemize}
\noindent Assumption \eqref{eq:ceofficients_constraints_2} is based on the fact that limit orders have the highest execution uncertainty, while market orders have the lowest, among the three order types.


See Table~\ref{tab:parameters_1} for the model coefficients we used for three different scenarios.
%\Jingwei{table updated}
\begin{footnotesize}
\begin{table}[htbp]
  \centering
  \caption{Model parameters used for the synthetic experiments}
    \begin{tabular}{ccccccc}
    \toprule
    \multicolumn{7}{c}{Scenario I ($d=4$)} \\
    \midrule
    $p$ & 0.1316 & 0.3218 & 0.5800 & 0.7367 &    &  \\
    $\sigma^2$ & 0.2506 & 0.2902 & 0.5090 & 0.7706 &    &  \\
    \midrule
    \multicolumn{7}{c}{Scenario II ($d=5$)} \\
    \midrule
    $p$ & 0.1121 & 0.2742 & 0.4942 & 0.5232 & 0.6278 &  \\
    $\sigma^2$ & 0.2318 & 0.2685 & 0.3798 & 0.4709 & 0.7129 &  \\
    \midrule
    \multicolumn{7}{c}{Scenario III ($d=6$)} \\
    \midrule
    $p$ & 0.1081 & 0.2641 & 0.2645 & 0.4767 & 0.5047 & 0.6055 \\
    $\sigma^2$ & 0.1631 & 0.1889 & 0.2672 & 0.3313 & 0.5015 & 0.7106 \\
    \end{tabular}%
  \label{tab:parameters_1}%
\end{table}%
\end{footnotesize}

\noindent{\bf Implementation Details:} We note that when implementing \rise, rather than strictly following \eqref{eq:n_a} and \eqref{eq:n} to decide the length of exploration phase,  we set $n = \lceil d T^{2/3} \rceil$ in the experiments for practical convenience.
Also, when implementing \risepp,  we set 
$$
n_{\ell, a} = \left\lceil 0.0001 \cdot \frac{d^{3}  \log(d) Q_{\ell}^{*} (a) }{\varepsilon_{\ell}^{2}} \log^2 \left( K T^2  \right)\right\rceil
$$ 
rather than strictly follow \eqref{eq:phase_elimination_phase_length}.
Moreover, we regularize the design matrix as $ V_{(\ell)}=\sum_{a \in \mathcal{A}_{\ell}} n_{\ell,a}  a a^{\top} + I_d $ to avoid singularity issue for \risepp. % rather than using $ V_{(\ell)}=\sum_{a \in \mathcal{A}_{\ell}} n_{\ell,a}  a a^{\top}$ ,


\noindent{\bf Criterion and Benchmark Algorithms:} In view of the connection between proxy regret and intermediate regret established in Proposition~\ref{prop:regret_trans}, we use the intermediate regret as a performance measure of different algorithms. 

We compare \rise~and \risepp~with two algorithms proposed by \cite{sani2012risk} for the MAB problem. 
The first one is a variation of the UCB policy (referred to as UCB(MAB)) and the second is a variation of the exploration-and-exploitation policy (referred to as ExpExp(MAB)).  To apply these two algorithms to the SOR problem, we simply let all non-negative integer allocations of $S$ orders into $d$ venues be the whole action space.  The implementations of the UCB(MAB) and ExpExp(MAB) strictly follow the descriptions in  \cite{sani2012risk}. 


\begin{figure}[!ht]
	\centering
	\subfigure[$d=4, S=4, K=35$ (Scenario I).]{\includegraphics[width=8cm,height=5.5cm]{plots/d=4,S=4.png} \label{fig:1_d4S4} }
	\subfigure[$d=5, S=4, K=70$ (Scenario II).]{\includegraphics[width=8cm,height=5.5cm]{plots/d=5,S=4.png} \label{fig:2_d5S4}	}
	\subfigure[$d=6, S=4, K = 126$ (Scenario III).]{\includegraphics[width=8cm,height=5.5cm]{plots/d=6,S=4.png} \label{fig:3_d6S4}	}
	\subfigure[$d=6, S=8, K=1287$ (Scenario III).]{\includegraphics[width=8cm,height=5.5cm]{plots/d=6,S=8.png} \label{fig:4_d6S8}	}
	\caption{Intermediate regrets of different algorithms over $T$. \rise~and \risepp~outperform the benchmark algorithms. }
	\label{fig:intermediate_regret}
\end{figure}


\noindent{\bf Numerical Performance and Discussion:} 
We provide one plot for scenario I (cf. Figure \ref{fig:1_d4S4}), one plot for scenario II (cf. Figure \ref{fig:2_d5S4}), and two plots for scenario III with different $S$ values (cf. Figures \ref{fig:3_d6S4}- \ref{fig:4_d6S8}).
First of all, it is evident that \rise~and \risepp~have the best empirical performances in all three different scenarios. 
Next, we observe in Figure~\ref{fig:1_d4S4} and \ref{fig:2_d5S4} that when action space is relatively small ($K=35$ or $K=70$), the UCB(MAB) still exhibits a logarithmic regret growth rate. 
It may outperform other three algorithms eventually, but its performance is the worst in the time frame we considered.
% However, as the action space grows, in Figure~\ref{fig:2} ($K=70$), though the UCB(MAB)   
% The empirical findings are consistent with the theoretical results. 
%Recall that instance-dependent intermediate regret growth rate of UCB(MAB) is $O(K)$ (with log dependence in $T$) and the instance-independent intermediate regret growth rate of ExpExp(MAB) is $O(K T^{2/3})$. This reemphasizes that linear bandit is more sample efficient when the action space is large.

Furthermore, through Figure~\ref{fig:1_d4S4} to \ref{fig:4_d6S8}, the performances of both UCB(MAB) and ExpExp(MAB) get worse as $K$ grows. 
Figure~\ref{fig:4_d6S8}  shows that regrets of them grow linearly when the action space is large ($K=1287$). 
Specifically, since the length of its exploration phase is $K (T/14)^{2/3}$,  UCB(ExpExp) will  uniformly explore over the whole horizon when $K$ is large.  
{On the contrary, \rise~and~\risepp~are able to fully utilize the linear structure of the problem and their regret growth rates do not rely on $K$, the size of action space. 
Therefore, \rise~and \risepp~are especially competent for tasks with a huge action space. 
However, the performance comparison between \rise~and \risepp~is more complex, which may depend on specific instances. 
}
\iffalse
\begin{figure}[htbp] 
  \begin{minipage}{\linewidth}
    \makebox[.5\linewidth]{\includegraphics[width=.45\linewidth]{plots/d=4,S=4.png}}%
    \makebox[.5\linewidth]{\includegraphics[width=.45\linewidth]{plots/d=5,S=4.png}}

    \makebox[.5\linewidth]{\small (a) $d=4, S=4, K=35$ (Scenario I).}%
    \makebox[.5\linewidth]{\small (b) $d=5, S=4, K=70$ (Scenario II).}%

    \medskip

    \makebox[.5\linewidth]{\includegraphics[width=.45\linewidth]{plots/d=6,S=4.png}}%
    \makebox[.5\linewidth]{\includegraphics[width=.45\linewidth]{plots/d=6,S=8.png}}

    \makebox[.5\linewidth]{\small (c) $d=6, S=4, K = 126$ (Scenario III).}%
    \makebox[.5\linewidth]{\small (d) $d=6, S=8, K=1287$ (Scenario III).}%
  \end{minipage}%
  \caption{Intermediate regrets of different algorithms over $T$.}
  \label{fig:numerical_regret}
\end{figure}
\fi 

\iffalse
\Ruihao{ 2 by 2 }
\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.6\linewidth]{plots/d=4,S=4.png}
  \caption{$d=4, S=4, K=35$ (Scenario I).}
  \label{fig:1_d4S4}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.6\linewidth]{plots/d=5,S=4.png}
  \caption{$d=5, S=4, K=70$ (Scenario II).}
  \label{fig:2_d5S4}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.6\linewidth]{plots/d=6,S=4.png}
  \caption{$d=6, S=4, K = 126$ (Scenario III).}
  \label{fig:3_d6S4}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.6\linewidth]{plots/d=6,S=8.png}
  \caption{$d=6, S=8, K=1287$ (Scenario III).}
  \label{fig:4_d6S8}
\end{figure}

\fi 

\subsection{A Numerical Study Based on the NASDAQ ITCH Dataset}\label{sec:study_realdata}
Undoubtedly, the actual performance of algorithms is susceptible to the environment specification. 
In this section, we conduct a numerical study using the NASDAQ ITCH dataset to extract model parameters and evaluate the assumptions made in the framework. 
This approach ensures that the results of our study are representative of actual financial decision-making scenarios, and can be used to make more informed decisions in practice.
%the results reflect real-world financial scenarios and can inform practical decision-making.
% By using real data, we can ensure that the results of our study are representative of actual financial decision-making scenarios and can be used to make more informed decisions in practice.

% In this section, we perform a numerical study where the model parameters are extracted from real financial data. In addition, the assumptions made in the framework are well justified by the data. 

\noindent{\bf Data Source:} 
Our numerical study is based on historical order book messages from three exchanges at NASDAQ on March 27, 2019.
The data is publicly available \citep{data}.
We only use data from 11:00 to 13:00, since the market is usually more stable during this period of time. 
We reconstruct the LOB % (with five best bid and ask quotes) 
from the message-level data using tools developed by \cite{https://doi.org/10.5281/zenodo.5209267}. 
We call the configuration of the LOB at a particular moment the \textit{snapshot} of the LOB. 
Each snapshot contains five queues on both the ask and bid side.
This dataset consists of 3 lit-pool venues: NASDAQ BX (BX), NASDAQ PSX (PSX) and The Nasdaq Stock Market (NASDAQ). 
Each of them is a stock exchange with different liquidity incentives. 
To be specific, NASDAQ has the conventional price/time matching mechanism, while PSX uses a price/pro-rata allocation rule and BX has an inverted pricing model. 
More details can be found at \eg, \cite{bx, psx, tradetalk}.  

\noindent{\bf Liquidity Simulation:}
We proceed to explain how we generate reasonable parameters in Eq.~\eqref{eq:sor_mean_model} and \eqref{eq:sor_var_model}  for lit pools and dark pools respectively. 
Primarily, we estimate the parameters for market orders of lit pools by an ``eat-up bid queues'' sampling procedure (to be explained shortly), then we  set parameters for dark pools in accordance with Assumptions~\eqref{eq:ceofficients_constraints_1} and \eqref{eq:ceofficients_constraints_2}.
Also, we assume that our task consists of selling $S$ shares of stocks every 2 minutes. 

The sampling procedure for estimation works as follows. 
For a given stock, we group all the LOB snapshots from 11:00 to 13:00 to 60 2-min buckets.
To estimate the PnL of submitting market orders to venue $j$, we sample uniformly \textit{over time} one snapshot at each venue $j$ from each bucket, with different values of \textit{test quantity} $Q^j$. 
Let $p^{\texttt{bid}, j}_{t, i}$ be the $i$th best bid price on the LOB snapshot at time $t$, and let $\bar{q}^{\texttt{bid}, j}_{t, i}$ be the corresponding queue size. 
We split $Q^j$ orders to the five queues, with as many orders to the more favorable prices as possible. 
To be precise,  let $q^{\texttt{bid}, j}_{t, i} \in [0, \bar{q}^{\texttt{bid}, j}_{t, i}]$ be the size of the market order submitted to the $i$th queue. 
We have $\sum_{i=1}^{5} q^{\texttt{bid}, j}_{t, i} = Q^j$.
Also, $ q^{\texttt{bid}, j}_{t, i} > 0 $ only when $ \sum_{i'=1}^{i - 1} q^{\texttt{bid}, j}_{t, i'} < Q^j$ for $ 2 \leq i \leq 5$.
Note that due to the nature of the problem, we do not need to set $Q^j$ too large so that the orders in the bid queues are not enough to fulfill. 
We denote $p^{\texttt{mid-price}, j }_{t}$ the mid-price of the $j$th venue.
Then the {\it relative} PnL of market orders is defined to be
\begin{equation} \label{eq:estimation_p}  %  \frac{1}{Q^j }  
   \sum_{i=1}^{5} p^{\texttt{bid}, j}_{t, i} q^{\texttt{bid}, j}_{t, i}  -  p^{\texttt{mid-price}, j }_{t} \cdot Q^j,
\end{equation}
against the benchmark level $p^{\texttt{mid-price}, j }_{t} \cdot Q^j$. See Figure~\ref{fig:bucket_lob} for visualization. 

To sample uniformly over time % rather than over events (changes of the limit order book), \renyuan{is it necessary to mention "rather than over events (changes of the limit order book)"? I would suggest deleting this half of the sentence.}
% the difference between profits from selling $S$ shares by eating up the bid queues, and profits from selling $S$ shares of stocks at the mid-price (which serves as the benchmark). 
we first uniformly sample a time point in the bucket, and then match it with the closest snapshot within the bucket. 
We note that this sampled time point is used across three venues. 
Finally, we obtain the empirical mean and variance PnL (cf. Eq.~\eqref{eq:estimation_p}) over 60 buckets.
% take average over 60 buckets to get one sample of estimated standardized trading price \renyuan{which standardized trading price? be more specific and use formulas. what is the connection to \eqref{eq:estimation_p}?}. 
%We repeat 100 samples to obtain the empirical mean and variance.


\begin{figure}[htbp]
    \centering
    \includegraphics[width=15cm]{plots/bucket_lob.png}
    \caption{Visualization of the sampling procedure. We sample one snapshot of the LOB from each bucket uniformly over time. Then we obtain the empirical mean and variance PnL (cf. Eq.~\eqref{eq:estimation_p}) over 60 buckets. 
     }
    \label{fig:bucket_lob}
\end{figure}

For dark pools, we do not have access to any data to simulate from. 
So based on the estimated first two moments ({\it i.e.}, mean and variance) of lit pools, we randomly generate moments of dark pools which satisfy Assumptions~\eqref{eq:ceofficients_constraints_1} and~\eqref{eq:ceofficients_constraints_2}.
Also, we make sure that the first two moments of dark pools are on a scale comparable to the lit pools. 
For this experiment, we set to sell $S=10$ shares over $d=5$ venues. 
Table~\ref{tab:parameters_2} reports the parameters we used for our experiments. 
The unit PnL is the PnL defined in~\eqref{eq:sor_mean_model} divided by $Q^j$. 
The row $p$ stands for the mean of the unit PnL, and it is estimated by Eq.~\eqref{eq:estimation_p}.
The row $\sigma^2$ stands for the estimated variances of unit PnL. 


\iffalse

--- TSLA | BX | 10 ---
mean BX -6.619991166666677
var BX 13.485229581088692

 --- TSLA | PSX | 10 ---
mean PSX -8.227117166666652
var PSX 19.50418520435525

--- TSLA | NASDAQ | 10 ---
mean NASDAQ -0.4158968333333398
var NASDAQ 0.05065445421775091
\fi


\begin{table}[htbp] 
  \centering
  \caption{Model parameters used for the experiment}
    \begin{tabular}{cccccc}
    \toprule
          & BX    & PSX   & NASDAQ & Dark pool 1 & Dark pool 2 \\
    \midrule
    $p$   & -0.662  & -0.823  &  -0.0416  & 0.05    & 0.001 \\
    $\sigma^2$  & 1.35  & 1.951    & 0.00507  & 2.1    & 2.3 \\
    \bottomrule
    \end{tabular}%
  \label{tab:parameters_2}%
\end{table}%

\begin{figure}[h]
	\centering
	\subfigure[BX  mean with R-squared $R^2=0.99$]{\includegraphics[width=8cm,height=5.5cm]{plots/BX_TSLA_mean.png} \label{fig:BX_TSLA_mean} }
	\subfigure[BX  var with R-squared $R^2=0.94$]{\includegraphics[width=8cm,height=5.5cm]{plots/BX_TSLA_var.png} \label{fig:BX_TSLA_var}	}
	\subfigure[PSX  mean with R-squared $R^2=0.99$]{\includegraphics[width=8cm,height=5.5cm]{plots/PSX_TSLA_mean.png} \label{fig:PSX_TSLA_mean}	}
	\subfigure[PSX  var]{\includegraphics[width=8cm,height=5.5cm]{plots/PSX_TSLA_var.png} \label{fig:PSX_TSLA_var with R-squared $R^2=0.94$}	}
	\subfigure[NASDAQ  mean with R-squared $R^2=0.99$]{\includegraphics[width=8cm,height=5.5cm]{plots/NASDAQ_TSLA_mean.png} \label{fig:NASDAQ_TSLA_mean} }
	\subfigure[NASDAQ  var with R-squared $R^2=0.93$]{\includegraphics[width=8cm,height=5.5cm]{plots/NASDAQ_TSLA_var.png} \label{fig:NASDAQ_TSLA_var}	}
	\caption{
 % Means and variances of standardized trading prices against $S$ for TSLA at different venues. 
 % We can see the fitness of a linear approximation varies across venues. 
 % The linear approximation works for NASDAQ best, while BX and PSX exhibit a piece-wise linear pattern. (which is unit PnL times  different values of test quantities $Q^j$)
The estimated means and variances of PnL for Tesla stock at different venues, as $Q^j$ varies.
 % Means and variances of unit PnL (cf. Eq.~\eqref{eq:estimation_p} times $S$, as $S$ varies for TSLA at different venues.
A clear linear relationship prevails for mean and a linear relationship for variance roughly holds.
This is an empirical justification for our linear form approximation Eq.~\eqref{eq:sor_mean_model} and Eq.~\eqref{eq:sor_var_model}. 
 }
	\label{fig:tsla}
\end{figure}

\noindent\textbf{Validation of Linearity:}
Figure~\ref{fig:tsla} plots the estimated means and variances of PnL for Tesla stock at different venues, as $Q^j$ varies.
We observe strong empirical evidence for a linear relationship between the mean trading profit and $Q^j$ for the considered scale of $Q^j$, which supports the approximation in Eq.~\eqref{eq:sor_mean_model}.
For modest values of $Q^j$ (such as $Q^j \sim 1 \times 10$ in our study), there is roughly a linear relationship between the variance of trading profit and $Q^j$. 
Essentially, this linearity critically hinges on the fact that we are trading a volume that will not eat up the best bid queue in a liquid market. % {\color{red}[I don't understand the last sentence. you mean ``eat up the queue?'']}

% We observe that the fitness of a linear approximation varies across venues. 
% The linear approximation works for NASDAQ best, while BX and PSX exhibit a piece-wise linear pattern. 



\noindent{\bf Numerical Performance:}
Figure~\ref{fig:tsla_regret} shows that \rise~and \risepp~still exhibit a sublinear regret growth in this more realistic experiment. 
Both \rise~and \risepp~will settle on the NASDAQ venue sooner or later.
Interestingly, we find that UCB(MAB) also performs quite well in this example. 
ExpExp(MAB) suffers a linear regret because its designed exploration phase scales as $K$, which will be excessively long in this case. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=10cm]{plots/TSLA.png}
    \caption{Intermediate regret. \rise~and \risepp~exhibit sublinear regret in the experiment based on the NASDAQ ITCH dataset. }
    \label{fig:tsla_regret}
\end{figure}



\newpage 



==> time_machine/sec_risepp_first_submission.tex <==

\section{Risk-Aware Successive Elimination (\texttt{RISE++}) Algorithm}
\label{sec:risepp}

In the previous section, \rise~is shown to be able to ensure a regret of $\tilde{O} \left( d T^{2/3} \right)$ for any underlying parameters of our problem. However, as already noticed in the MAB setting (see, \eg, Section 7 of \cite{lattimore2020bandit}), it is in fact possible to attain a much smaller regret (in terms of dependence on $T$) when the problem parameters are set in favor of learning (especially when $\Delta_a$'s are relatively large when compared to $1/T$). 

In this section, we exploit this possibility for risk-aware linear bandits. We first introduce the Risk-Aware Successive Elimination (\risepp) algorithm, and then establish its instance-dependent regret upper bound.

\subsection{The Algorithm}
\noindent\textbf{Additional Notations:} 
Let $C_4$ be the leading constant prescribed in Eq.(17) in \cite{stay2019}. 
Let $\hat{C}$ be a constant which ensures that 
$$
 8 \rho    \sigma_{\max }^{2} \sqrt{d + \log \left( 2 T^2 \delta^{-1} \right)} + C_4   d \sqrt{\log(d)}  \log(T \delta^{-1} )   \leq \hat{C} d\sqrt{\log(d)} \log\left(T \delta^{-1} \right). 
$$

\noindent\textbf{Algorithm:} 
The \underline{Ri}sk-Aware \underline{S}uccessive \underline{E}limination (\texttt{RISE++}) algorithm successively eliminates undesirable actions in phases. 
In each phase, the remaining actions are explored in accordance with a G-optimal design. 

To be specific, in phase $\ell$ for $\ell = 1, 2, \cdots$, let $\mathcal{A}_{\ell}$ be the set of promising actions to explore. We initialize $\mathcal{A}_{1}$ to be $\mathcal{A}$. 
In each phase, a new exploration basis is identified using the G-optimal design distribution $Q^{*}_{\ell}$, which is the solution to the following minimization problem:
\begin{align}
    \nonumber&\underset{Q(\cdot)}{\operatorname{minimize}} ~g_{\ell}(Q):=\max_{x\in\cA_{\ell}}~x^{\top}\left(\sum_{a\in\cA_{\ell}} Q(a)aa^{\top}\right)^{-1}x\\
    &\text{s.t.,}~\sum_{a\in\cA}Q(a)=1\,,\ Q(a)\geq 0~\forall a\in\cA_{\ell}.  \label{eq:phase_elimination_g_optimal_design}
\end{align}
Then, the algorithm selects each action $a \in \mathcal{A}_{\ell}$ by 
\begin{equation} \label{eq:phase_elimination_phase_length}
    n_{\ell,a}=\left\lceil \hat{C}^2 \frac{d^{2} g_{\ell}(Q_{\ell}^{*}) \log(d) Q_{\ell}^{*} (a) }{\varepsilon_{\ell}^{2}} \log^2 \left(\frac{ K T }{\delta}\right)\right\rceil 
\end{equation}
number of times, where $\delta$ is an input parameter and $\varepsilon_{\ell}=2^{- \ell}$ is the tolerance level in phase $\ell$.
We denote by $n_{(\ell)} = \sum_{a \in \mathcal{A}_{\ell} } n_{\ell,a}$ the length of phase $\ell$.
Let $ V_{(\ell)}=\sum_{a \in \mathcal{A}_{\ell}} n_{\ell,a}  a a^{\top}$ be the design matrix used in phase $\ell$. 
Let $t_{\ell}$ be the timestep of the beginning of phase $\ell$. 
Next, parameters $\theta_{*}$ and $\phi_{*}$ are estimated by OLS estimators
\begin{equation} \label{eq:phase_elimination_theta_hat}
    \hat{\theta}_{(\ell)}=V_{(\ell)}^{-1} \sum_{t=t_{\ell}}^{t_{\ell}+n_{(\ell)}} A_{t} X_{t}  
\end{equation}
and 
\begin{equation} \label{eq:phase_elimination_phi_hat}
\hat{\phi}_{(\ell)} = V_{(\ell)}^{-1} 
\sum_{t= t_\ell}^{ t_{\ell} +n_{(\ell)} } f^{-1} \left(\left( X_t - \inner{\hat{\theta}_{(\ell)} , A_t} \right)^2 \right) A_t . 
\end{equation}

Underperforming actions are eliminated based on these estimates with the tolerance level $\varepsilon_{\ell}$.
Thus,  the action set to explore for phase $\ell + 1$ is 
\begin{equation} \label{eq:phase_elimination_new_action_set}
\mathcal{A}_{\ell+1}=\left\{a \in \mathcal{A}_{\ell}: \max_{b \in \mathcal{A}_{\ell}}~\left\langle
\rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)}
, b-a\right\rangle \leq 2 \varepsilon_{\ell}\right\} .
\end{equation}
The formal description of the \rise~algorithm is presented in Algorithm \ref{algo:phase_ elimination}.

% \Jingwei{2024/12/01: There is a technical flaw we need to fix: since we eliminate arms gradually, we need to make sure the design matrix is still invertible. We can accomplish this by at least two ways: (1) projections to a lower dimension; (2) add a regularization. We need to add a rigorous argument for the latter. 
% }

\begin{algorithm}[htbp]
  \caption{Risk-Aware Successive Elimination Algorithm.} \label{algo:phase_ elimination}
  \begin{algorithmic}[]
  \footnotesize 
    \State Set $\ell = 1$, and $\mathcal{A}_1 = \mathcal{A}$.
\While { true  }
    \State (1) Given $\mathcal{A}_{\ell}$, find the G-optimal design $Q^*_{\ell}$ following % \eqref{eq:phase_elimination_g_optimal_design}.
\begin{align}
    \nonumber&\underset{Q(\cdot)}{\operatorname{minimize}} ~g_{\ell}(Q):=\max_{a\in\cA_{\ell}}~ x^{\top}\left(\sum_{a\in\cA_{\ell}} Q(a)aa^{\top}\right)^{-1} x \nonumber \\
    &\text{s.t.,}~\sum_{a\in\cA}Q(a)=1\,,\ Q(a)\geq 0~\forall a\in\cA_{\ell}. \nonumber  
\end{align}
    \State (2) Select each action $a \in \mathcal{A}_{\ell}$ for $$n_{\ell,a} = \left\lceil \hat{C}^2 \frac{d^{2} g_{\ell}(Q_{\ell}^{*}) \log(d) Q_{\ell}^{*} (a) }{\varepsilon_{\ell}^{2}} \log^2 \left(\frac{ K T }{\delta}\right)\right\rceil  $$ times. % , where $n_{\ell,a}$ is defined as %  \eqref{eq:phase_elimination_phase_length}. 
    \State (3) Compute least squares estimates according to % \eqref{eq:phase_elimination_theta_hat} and \eqref{eq:phase_elimination_phi_hat} .
\begin{eqnarray*}
\hat{\theta}_{(\ell)}&=&V_{(\ell)}^{-1} \sum_{t=t_{\ell}}^{t_{\ell}+n_{(\ell)}} A_{t} X_{t} ,  \\ 
\text{ and  } \hat{\phi}_{(\ell)} &=& V_{(\ell)}^{-1} 
\sum_{t= t_\ell}^{ t_{\ell} +n_{(\ell)} } f^{-1} \left(\left( X_t - \inner{\hat{\theta}_{(\ell)} , A_t} \right)^2 \right) A_t . 
\end{eqnarray*}
    \State (4) Eliminate underperforming actions in terms of MV according to 
$$
\mathcal{A}_{\ell+1}=\left\{a \in \mathcal{A}_{\ell}: \max _{b \in \mathcal{A}_{\ell}}\left\langle
\rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)}
, b-a\right\rangle \leq 2 \varepsilon_{\ell}\right\} .    
$$
    % \eqref{eq:phase_elimination_new_action_set}. 
    \State (5) $\ell = \ell + 1 $.
\EndWhile
\end{algorithmic}
\end{algorithm}


\begin{remark}[\textbf{Comparisons with the Design of \rise}]
Although it is evident that the design of \risepp~shares some similarities with \rise~(\eg, both of them are driven by the variance-minimizing G-optimal design), there are several critical differences: 
(1) \risepp~could have potentially more than one phase and keeps eliminating underperforming actions as long as there is more than one action remaining. Meanwhile, \rise~only permits a single phase; 
(2) Associated with the previous point, \risepp~has to re-compute the G-optimal design (\textit{w.r.t.} the remaining actions) at the beginning of each phase. 
In contrast, \rise~only needs to compute the G-optimal design once. Altogether, one can immediately conclude that \risepp~virtually never stops exploration (as long as there are more than one action left).  
As shown in the forthcoming Theorem~\ref{thm:risepp_regret}, this is extremely critical in achieving low instance-dependent regret. The reason is that the continuously exploring nature of \risepp~prevents it from stopping prematurely (as what \rise~might), and can truly exploit the benign problem parameters.
\end{remark}


\Jingwei{I still think we need to address the invertibility issue of the design matrix. 
Chapter 22 in \cite{lattimore2020bandit} completely ignores this issue and I believe it is problematic.
}

\Jingwei{@ Renyuan and Ruihao: start line of new material}

\subsection{Regret Analysis}
% Denote $\bar{\mu}_a(T) = \frac{1}{ \sum_{t=1}^{T} \one{A_t=a} } \sum_{t=1}^{T} \one{A_t=a} X_t $.
% To bound the expected regret of \risepp, we first invoke the following result.
% Though it was derived in the MAB context, one can easily verify that it carries over to our linear bandit setting. 
% \Jingwei{The term $\tau_a (T) $ in eq. (25) that denotes the total number of times of pulling an arm
% a is not explicitly defined.}
% \begin{proposition}[Lemma 2 in \cite{vakili2016}] \label{lemma:vakili_regret_decomposition}
% The expected regret can be decomposed as 
% \begin{align}\label{eq:lemma_vakili_regret_decomposition}
% \nonumber \E{\reg_{\pi}(T)} = &\sum_{a \in \mathcal{A} }^{} \mathbb{E}\left[\tau_{a}(T)\right] \Delta_{a}
% + \sum_{a \in \mathcal{A}}^{} \mathbb{E}\left[\tau_{a}(T)\right] \Gamma_{a, *}^{2}-\frac{1}{T} \mathbb{E}\left[\left(\sum_{a \in \mathcal{A}}^{} \tau_{a}(T)\left(\bar{\mu}_{a}(T) - \mu_{*} \right)\right)^{2} \right]+\sigma_{*}^{2}\\
% \leq&\sum_{a \in \mathcal{A} }^{} \mathbb{E}\left[\tau_{a}(T)\right] (\Delta_{a}+\Gamma_{a, *}^{2})  +\sigma_{*}^{2}\,.
% \end{align}
% \end{proposition}
% Given the decomposition of the expected regret, it suffices to bound the expected number of times to pull a suboptimal action.
Our proof strategy is to conduct a careful analysis of the algorithm based on the temporal decomposition Proposition~\ref{prop:temporal_decomposition}. 
It turns out that by carefully examining the behavior of \risepp, we can provide a tighter bound on a term which we could only bound by $O(\sqrt{T})$ for a generic algorithm.  


To proceed, we first need to quantify how well \risepp~keeps refining its estimates of MVs of each action over the entire horizon.

\begin{proposition}
\label{lemma:phase_elimination_confidence_bound_theta_phi_any_t}
For any $\delta > 0$, we have 
\begin{equation}
   \p {
    \left | \inner{ \rho \theta_{*} - \phi_{*} - \left( \rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)} \right) , a } \right | 
    \leq \varepsilon_{\ell},~ \forall~ a \in \mathcal{A}, ~ \forall~\ell \in \mathbb{N}
    } \geq 1 - \delta .
\end{equation}
\end{proposition}
The proof of this proposition is provided in Online Companion \ref{sec:proof_prop_phase_elimination_confidence_bound_theta_phi_any_t}.
Note that Proposition~\ref{lemma:phase_elimination_confidence_bound_theta_phi_any_t} is a variation of Proposition~\ref{prop:bound_ip}, being more convenient to use for the analysis of \risepp.

With underperforming actions removed in each phase, we can show that with high probability, a suboptimal action $a$ with gap $\Delta_a$ will be eliminated before phase $\ell_a = \min \{\ell \geq 1: 2 \varepsilon_\ell < \Delta_a  \} = \lceil \log_2(2 / \Delta_a ) \rceil$.
Denote 
$
\Delta = \underset{a \in \mathcal{A}, ~a \neq a_*  }{\min} ~ \Delta_a \ .
$
With high probability, after $\bar{t}$ periods, there is only one arm left, where 
\begin{eqnarray}
    \bar{t}  &=&  \sum_{\ell = 1}^{ \lceil \log_2(2 / \Delta ) \rceil }  
    n_{(\ell)}   \ . 
\end{eqnarray}
% We remark that this quantity may exceed $T$. 
By exploiting this fact, we can refine the \( O\paren{\sqrt{T}} \) term in Proposition~\ref{prop:temporal_decomposition}, which accounts for the variance arising from the interaction between future actions and current noise. 
Although we can only guarantee an \( O\paren{\sqrt{T}} \) bound over this term for a \textit{generic} algorithm, the analysis simplifies on the event that the algorithm pulls only a single arm, allowing us to achieve a much sharper estimate.
We manage to prove the following theorem. 


% When event $G$ happens, all suboptimal arms except $a_*$ are eliminated before phase $\lceil \log_2(2 / \Delta ) \rceil$. 
% After that, only the action $a_*$ remains. 
% Denote by $\bar{t}$ the time after which there is only one arm left. Namely, 

% the MV gap of a suboptimal action chosen in phase $\ell$ is at most $2 \varepsilon_{\ell}$. 
% In other words, with high probability, a suboptimal action $a$ with gap $\Delta_a$ will be eliminated before phase $\ell_a = \min \{\ell \geq 1: 2 \varepsilon_\ell < \Delta_a  \} = \lceil \log_2(2 / \Delta_a ) \rceil$. 
% By properly tuning the parameter $\delta$ for \risepp, we can bound the expected number of times a suboptimal action being pulled. 

% \begin{proposition} \label{lemma:phase_elimination_pulled_times_upper_bound}
% With $\delta=T^{-1}$, the expected number of times a suboptimal action $a \neq a_*$ with gap $\Delta_a > 0$ being pulled by \risepp~is upper bounded by 
% \begin{equation}\label{eq:upper_bound_tau}
%     \E{\tau_a(T)} \leq  O \left(  \frac{ d^{3} \log(d) \log^2(K T)}{\Delta^2_a}  \left( \sum_{\ell=1}^{\ell_a}  Q^*_{l}(a) \right)   \right) . 
% \end{equation}
% \end{proposition}
% The proof of this proposition is provided in Online Companion~\ref{sec:proof_prop_phase_elimination_pulled_times_upper_bound}.

% Combining Proposition~\ref{lemma:vakili_regret_decomposition} and Proposition~\ref{lemma:phase_elimination_pulled_times_upper_bound}, and defining $\ell_{\max}$ as the maximum number of phases, we can derive that the expected regret of \risepp~is
% \begin{align}
%     \nonumber\E{\reg_{\risepp}(T)} =& O \left(\sum_{a\in\cA}  \frac{ d^{3} \log(d) \log^2(K T)(\Delta_{a}+\Gamma_{a, *}^{2}) }{\Delta^2_a}  \left(\sum_{\ell=1}^{\ell_a}  Q^*_{l}(a)\right) \right)\\
%     \nonumber= &O \left(\max_{a\in\cA} \left(\frac{ \Delta_{a}+\Gamma_{a, *}^{2} }{\Delta^2_a}\right)d^{3} \log(d) \log^2(K T)  \left(\sum_{a\in\cA}\sum_{\ell=1}^{\ell_a}  Q^*_{l}(a)\right)  \right)\\
%    \nonumber= &O \left(\max_{a\in\cA} \left(\frac{ \Delta_{a}+\Gamma_{a, *}^{2} }{\Delta^2_a}\right)d^{3} \log(d) \log^2(K T)  \left(\sum_{a\in\cA}\sum_{\ell=1}^{\ell_{\max}}  Q^*_{l}(a)\right) \right)\\
%    = & O \left(\max_{a\in\cA} \left(\frac{ \Delta_{a}+\Gamma_{a, *}^{2} }{\Delta^2_a}\right)d^{3} \log(d) \log^2(K T^{2}) \log(T) \right) \,. \label{eq:proxy_regret_new}
% \end{align}
% The second equation follows as we take the maximum over $a$ for the term $(\Delta_a+\Gamma^2_{a,*})/\Delta^2_a\,.$ The last equation follows because $$ \sum_{a\in\cA}\sum_{\ell=1}^{\ell_{\max}}  Q^*_{l}(a) = \sum_{\ell=1}^{\ell_{\max}} \sum_{a\in\cA}  Q^*_{l}(a) = \ell_{\max}= O \left( \log(T) \right). $$ 
% Indeed, the length of phase $\ell$ is at least $n_{(\ell)} = \sum_{a \in \mathcal{A}_{\ell}} \left\lceil \hat{C}^2 \frac{d^{2} g_{\ell}(Q_{\ell}^{*})  \log(d) Q_{\ell}^{*} (a) }{\varepsilon_{\ell}^{2}} \log^2 \left(\frac{ K T }{\delta}\right)\right\rceil  \geq \hat{C}^2 \frac{d^{3}  \log(d) }{\varepsilon_{\ell}^{2}} \log^2 \left(\frac{ K T }{\delta}\right) \,.$
% By setting $\sum_{\ell=1}^{\ell_{\max}} \hat{C}^2 {d^{3}  \log(d) }{\varepsilon_{\ell}^{-2}} \log^2 \left({ K T }/{\delta}\right) = T$ and $\delta=T^{-1}\,,$ 
% we thus have $$ \ell_{\max} = \frac{1}{2} \log \left( \frac{3 T}{\hat{C}^2 d^{3}\log(d) \log^{2}(KT^2) } \right) = O \left( \log(T) \right) \,.$$

% \iffalse
% \Jingwei{To be changed ----------------------------------------------}
% We note that the sum in \eqref{eq:proxy_regret_risepp} is over all actions selected by the G-optimal design in the first phase, with no more than $d(d+1)/2$ of them.  
% This is because by the construction of \risepp, the exploration basis in each phase is non-increasing in the sense that $\mathcal{A}_{\ell+1} \subset \mathcal{A}_{\ell}$. Hence, actions not selected in the first phase will not be taken later on. \Ruihao{This paragraph is incorrect. I have changed the derivation, $\ell_{\max}$ is the maximum number of phases, which should be $O(\log(T))$ (check this and then finish the rest)}

% Therefore, we have
% \begin{align} \label{eq:proxy_regret_new}
%     \E{\hat{R}_{\pi}(T)} 
%    = &O \left(\max_{a\in\cA} \left(\frac{ \Delta_{a}+\Gamma_{a, *}^{2} }{\Delta^2_a}\right)d^{3} \log(d) \log^3(K T^{2}) \right)\,.
% \end{align}

% \begin{proposition}[Theorem 1 in \cite{vakili2016}]
% For any policy $\pi$, we have 
% \begin{equation}
%     0 \leq \E{R_{\pi}(T) - \hat{R}_{\pi}(T)} \leq \sigma_{\max }^{2}\left(\sum_{i \neq *} \frac{\Gamma_{a, *}^{2}}{\Delta_{i}}+1\right)
% \end{equation}
% \end{proposition}
% \fi 
\begin{theorem}\label{thm:risepp_regret}
With $\delta=T^{-1}$, the expected regret of \risepp~is
% \begin{align*}
%     \E{\reg_{\risepp}(T)}= O \left(  
%     \max_{a\in\cA} \left(\frac{ \Delta_{a}+\Gamma_{a, *}^{2} }{\Delta^2_a}\right)d^{3} \log(d) \log^3(K T)
%     \right).
% \end{align*}
\begin{equation}
    \E{\reg_{\risepp}(T)} = O \paren{ \max_{a\in\cA} \left(\frac{ \Delta_{a}+\Gamma_{a, *}^{2} }{\Delta^2_a}\right)  d^3 \log(d) \log(T) \log^2 \left( K T^2 \right) + d^2 \log_2 \paren{\frac{1}{\Delta}} + d^2 \Delta }  \ . 
\end{equation}
\end{theorem}

\iffalse
Now we recall that it follows from Theorem 1 of \cite{vakili2016} that the difference between expected regret and expected proxy regret is bounded, \textit{i.e.} $\E{R_{\pi}(T) - \hat{R}_{\pi}(T)}  \leq \sigma_{\max }^{2} \cdot \left(1 + \sum_{a \neq a_*} {\Gamma_{a, *}^{2}}/{\Delta_{a}}\right)$.
Therefore, \eqref{eq:proxy_regret_new} can be translated to a bound of the expected regret, which we conclude in the following theorem. 
\begin{theorem}\label{thm:risepp_regret}
With $\delta=T^{-1}$, the expected regret of \risepp~is
\begin{align*}
    \E{R_{\pi}(T)}= O \left(  
    \sigma_{\max }^{2} \cdot \left(1+\sum_{a \neq a_*} \frac{\Gamma_{a, *}^{2}}{\Delta_{a}}\right) +
    \max_{a\in\cA} \left(\frac{ \Delta_{a}+\Gamma_{a, *}^{2} }{\Delta^2_a}\right)d^{3} \log(d) \log^3(K T)
    \right).
\end{align*}
\end{theorem}
Here, since the dominating terms in the regret upper bound is the logarithmic terms (\textit{w.r.t.} T), we use the $O(\cdot)$ notations for regret expressions instead of $\tilde{O}(\cdot)$ because the latter would hide the logarithmic terms.
\fi 

To this end, we make a couple of discussions to compare the regret bounds of prior works and that of \rise 's. 

\Jingwei{@ Professors: How and whether should we mention our old proof? }

\begin{remark}[\textbf{Comparisons with \cite{sani2012risk,vakili2016}}]
In view of the instance-dependent regret lower bound established in \cite{vakili2016}, we can conclude that our dependence on $T$ is nearly optimal up to a factor of $O(\log^2(T))$ (after ignoring dependence on $d$ and $K$). 
Moreover, compared to \cite{sani2012risk,vakili2016}, \risepp~decouples the two parameters $K$ and $T$, which makes it suitable for applications with large action sets. 
\end{remark}

\begin{remark}[\textbf{Comparisons with Instance-Independent Regret}]
We notice that the $O(d^3\log(d)\log^3(KT))$ instance-dependent regret bound can potentially provide an exponential improvement in terms of the dependence on $T$ when compared with the $\tilde{O} (d T^{2/3} ) $ instance-independent regret bound. Of course, there is a slightly worse dependence on $d\log(d)\,.$ This is expected as it is similar to the canonical MAB setting \citep{lattimore2020bandit}. Following the regret bounds, the benefits of instance-dependent regret becomes more obvious when $T$ grows large. This also aligns with prior understandings in the canonical MAB settings, that instance-dependent regret upper bounds become more meaningful when $\Delta$'s are relatively large when compared to $1/T.$ Nevertheless, we emphasize that, by taking advantage of the linear structure, both of them decouple the dependence on $K$ and $T$. 
\end{remark}

\Jingwei{@ Renyuan and Ruihao: end line of new material}



\subsection{New Patch }




Recalling the definition of $n_{\ell,a}$ in \eqref{eq:phase_elimination_phase_length}, we have 
\begin{eqnarray*}
 V_{(\ell)}= \lambda I + \sum_{a \in \mathcal{A}_{\ell}} n_{\ell,a} a a^{\top} &=&  \lambda I + \sum_{a \in \mathcal{A}_{\ell}  } \left\lceil \hat{C}^2 \frac{d^{3}  \log(d) Q_{\ell}^{*}(a)}{\varepsilon_{\ell}^{2}} \log^{2} \left(\frac{ K T }{\delta}\right)\right\rceil a a^{\top} \\
 &\succeq& \hat{C}^{2} \frac{ d^{3}  \log(d)}{\varepsilon_{\ell}^{2}} \log^{2} \left(\frac{ K T}{\delta}\right) \sum_{a \in \mathcal{A}_{\ell} }  Q_{\ell}^{*}(a) a a^{\top}    .  %  \preceq
 % &=& \hat{C}^{2} \frac{ d^{2} g(Q^{*}_{\ell}) \log(d)}{\varepsilon_{\ell}^{2}} \log^{2} \left(\frac{ K T}{\delta}\right) \sum_{a \in \mathcal{A}_{\ell}} Q^{*}_{\ell} (a) a a^\top    % V( Q_{\ell}^{*})
\end{eqnarray*}

Hence, by Lemma~\ref{lemma:A_geq_B}, we see that for any $a \in \mathcal{A}_{\ell}$, 
\begin{eqnarray}
  \left \| a \right\|_{V_{(\ell)}^{-1}} &=& \sqrt{ a^{\top} V_{(\ell)}^{-1} a }  \leq \frac{\varepsilon_{\ell}^{}}{\hat{C} d \sqrt{\log{d}}} \frac{1}{ \log \left(\frac{ K T}{\delta}\right)  } \sqrt{\frac{a^{\top} \left(  \sum_{a \in \mathcal{A}_{\ell} }  Q_{\ell}^{*}(a) a a^{\top} \right)^{\dagger} a}{d}  } \nonumber  \\
 &\leq&   \frac{\varepsilon_{\ell}^{}}{\hat{C} d \sqrt{\log{d}}} \frac{1}{ \log \left(\frac{ K T}{\delta}\right)  }    \label{eq:bound_inner_product_MV_preliminary_2} \ ,
\end{eqnarray}
where the last inequality follows from the fact that $Q^{*}_{\ell}(\cdot)$ is an optimal solution to \eqref{eq:phase_elimination_g_optimal_design}. 
By combining \eqref{eq:bound_inner_product_MV_preliminary_1} and \eqref{eq:bound_inner_product_MV_preliminary_2}, we conclude the desired result. 



Suppose $\operatorname{dim} (\operatorname{span} (A)) = m < d$. 
Let $B \in \mathbb{R}^{m \times d} $ be a matrix containing an orthonormal basis for $\operatorname{span}(\mathcal{A})$.
For every $a \in \mathcal{A}$, define $ \tilde{a} = B a$. Let $\tilde{\mathcal{A}}$ be the set that contains all such actions: 
\begin{equation}  
    \tilde{\mathcal{A}} = \braces{ \tilde{a} : \tilde{a} = B a, a \in \mathcal{A}  } \ . \nonumber
\end{equation}
We can apply G-optimal design on the set $\tilde{A}$. 
By General Equivalence Theorem of \cite{kiefer1960equivalence}, we can find a distribution $\tilde{\pi}^*$ supported on $\tilde{\mathcal{A}}$ such that 
\begin{equation}  \label{eq:max_self_normalized_aTilde}
      \max_{\tilde{a} \in \tilde{\mathcal{A}} } ~ \| \tilde{a} \|^{2}_{ \tilde{V}( \tilde{\pi}^* )^{-1} } = m \ , 
\end{equation}
where $\tilde{V}(\tilde{\pi}^*) = \sum_{\tilde{a} \in \tilde{\mathcal{A}}} \tilde{\pi}^*( \tilde{a} ) \tilde{a} \tilde{a}^{\top}$
and the size of support of $\tilde{\pi}^*$ is less than or equal to $\frac{m(m+1)}{2}$.

Given $\tilde{\pi}^*$, we can convert it to $\pi^*$, a distribution supported on $\mathcal{A}$ by the following procedure 
$$
   \pi^*(a) =
\begin{cases}
 \tilde{\pi}^* (\tilde{a})  , & \text{if } a \in \mathcal{A} \text{ and hence }  \tilde{a} = B a , \\
0 , & \text{otherwise } . 
\end{cases}
$$
Then we have 
$
V(\pi^*) = \sum_{a \in \mathcal{A}} \pi^* ( a ) a a^{\top} = \sum_{\tilde{a} \in \tilde{\mathcal{A}}} \tilde{\pi}^* (\tilde{a}) B^{\top} \tilde{a} \tilde{a}^{\top} B = B^{\top} \tilde{V}( \tilde{\pi}^* )  B  \ . 
$
Hence, $V(\pi^*)$ has pseudo-inverse $V(\pi^*)^{\dagger} = B^{\top}  \tilde{V}( \tilde{\pi}^* )^{-1}  B$. 
We further note that for every $a \in \mathcal{A}$, 
$$
\| a \|_{V(\pi^*)^{\dagger}}^{2}  = a^{\top} B^{\top} V(\tilde{\pi}^*)^{-1} B a = \tilde{a}^{\top} V(\tilde{\pi}^*)^{-1} \tilde{a} = \| \tilde{a} \|^{2}_{ \tilde{V}( \tilde{\pi}^* )^{-1} } \ . 
$$
Noting \eqref{eq:max_self_normalized_aTilde}, we conclude that 
$$
 \max_{a \in \mathcal{A}} ~ \| a \|_{V(\pi^*)^{\dagger}}^{2}   = m \ . 
$$




Now, when the action set $\mathcal{A}_{\ell}$ does not span $\mathbb{R}^d$, we need to use regularized estimators. Namely, we let 


\Jingwei{Need to include $\lambda$ in the following: }
\begin{eqnarray}
\left | \inner{ \rho \theta_{*} - \phi_{*} - \left( \rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)} \right) , a } \right | 
&\leq& 
\left \|  \rho \theta_{*} - \phi_{*} - \left( \rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)} \right) \right\|_{V_{(\ell)}} 
\left \| a \right\|_{V_{(\ell)}^{-1}} \nonumber \\
&\leq& \left (\rho \left \| \hat{\theta}_{(\ell)}-\theta_{*} \right \|_{V_{(\ell)}} + \left \| \hat{\phi}_{(\ell)}-\phi_{*} \right \|_{V_{(\ell)}} \right)  \left \| a \right \|_{V_{(\ell)}^{-1}} \nonumber \\
&\leq&  \left(  \rho   8 \sigma_{\max }^{2} \sqrt{d + \log \left(\frac{2 T^2 }{\delta }\right)} + C_4    d\sqrt{\log(d)}  \log(\frac{ T}{\delta })       \right)  \left \| a \right \|_{V_{(\ell)}^{-1}}    \nonumber \\ 
&\leq& \hat{C} d\sqrt{\log(d)} \log\left(\frac{ T}{\delta}\right) \left \| a \right\|_{V_{(\ell)}^{-1}}    % \log\left(\frac{T+\lambda}{\delta \lambda}\right)
\end{eqnarray}




$\hat{\theta} = , \hat{\phi} = $

































\iffalse
\subsection{Proof of Proposition~\ref{lemma:phase_elimination_pulled_times_upper_bound}}
\label{sec:proof_prop_phase_elimination_pulled_times_upper_bound}
We denote by $G_{\ell}^{a}$ the event that the MV estimate for action $a$ in phase $\ell$ deviates from the true value no more than $\varepsilon_{\ell}$, namely, 
$$
G_{\ell}^{a} = \left \{ \left| \inner{\rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)} - \left( \rho \theta_{*} - \phi_{*} \right), a } \right|  \leq \varepsilon_{\ell} \right \} .
$$
We say the \textit{good event} happens if for any action $a$ in exploration basis $\mathcal{A}_{\ell}$ in all phases, $G_{\ell}^{a}$ happens. 
\textit{I.e.}, we let 
$G = \underset{\ell}{\midcap} \underset{a \in \mathcal{A}_{\ell}}{\midcap} G_{a}^{\ell}$. 
By Lemma~\ref{lemma:phase_elimination_confidence_bound_theta_phi_any_t}, we know the event $G$ happens with probability at least $1 - \delta$. 

We first observe that if $G$ happens, then in phase $\ell$, the optimal action $a_{*}$ will not be eliminated at step (4) in Algorithm~\ref{algo:phase_ elimination}. 
To see this, suppose in phase $\ell$, the optimal action $a_{*}$ were eliminated by some suboptimal action $b$, which would mean $\exists~b \in \mathcal{A}_{\ell}$ such that 
\begin{eqnarray}
&& 
\inner{\rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)}, b-a_{*}} > 2 \varepsilon_{\ell} \nonumber  \\
 &\Leftrightarrow~& 
\langle \rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)}, b  \rangle - \varepsilon_{\ell} > 
\langle \rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)}, a_*  \rangle + \varepsilon_{\ell}. \label{eq:good_estimate_1}
\end{eqnarray}
Since $G$ happens, we have 
$$
\langle \rho \theta_{*} - \phi_{*}, b  \rangle \geq \langle \rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)}, b  \rangle - \varepsilon_{\ell}  ~~\text{and}~~ \langle \rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)}, a_*  \rangle + \varepsilon_{\ell} \geq \langle \rho \theta_{*} - \phi_{*}, a_*  \rangle
,$$
which, combined with \eqref{eq:good_estimate_1}, leads to the contradiction $\langle \rho \theta_{*} - \phi_{*}, b  \rangle >\langle \rho \theta_{*} - \phi_{*}, a_*  \rangle$.

%Next, we argue that when $G$ happens, the loss in stage $\ell$ from pulling an arm once is at most a constant times $\varepsilon_{\ell}$. 
Next, we argue that provided the good event $G$ happens, a suboptimal action $a$ with gap $\Delta_a$ will be eliminated before $\ell_a = \min \{\ell: 2 \varepsilon_\ell < \Delta_a \}$. 
Indeed, at step (3) of phase $\ell+1$, the estimated MV gap of action $a$ based on estimators in the previous phase $\ell$ is no more than  $2 \varepsilon_\ell$, \textit{i.e.}, 
$$
\max _{b \in \mathcal{A}_{\ell+1 }} \inner{ \rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)}, b-a } \leq 2 \varepsilon_{\ell} = 4 \varepsilon_{l+1}.
$$
In particular, the optimal action $a_*$ remains in $\mathcal{A}_{\ell+1}$. Hence, we have 
\begin{equation} \label{eq:1}
    \inner{ \rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)} , a_* - a } \leq 2 \varepsilon_{\ell}
\end{equation}
for any suboptimal action $a \in \mathcal{A}_{\ell+1}$.
On the other hand, the event $G$ implies that 
$-\varepsilon_{\ell}   \leq \inner{ \rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)} - \left( \rho \theta_{*} - \phi_{*} \right) , a  } \leq \varepsilon_{\ell}$ 
and $-\varepsilon_{\ell} \leq \inner{  \rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)} - \left( \rho \theta_{*} - \phi_{*} \right), a_*  } \leq \varepsilon_{\ell}$ hold, which means    
% $$
% - 2\varepsilon_{\ell} \leq \inner{  \rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)} - \left( \rho \theta_{*} - \phi_{*} \right) , a_* - a  } \leq % 2\varepsilon_{\ell},
% $$
% which is equivalent to 
\begin{equation} \label{eq:2}
  -2\varepsilon_{\ell} \leq 
\inner{ \rho \theta_{*} - \phi_{*}  , a_* - a  } 
- \inner{ \rho \hat{\theta}_{(\ell)} - \hat{\phi}_{(\ell)} , a_* - a  }
\leq 2\varepsilon_{\ell}. 
\end{equation}
Combining \eqref{eq:1} and \eqref{eq:2} yields that 
$$
\Delta_a = \inner{ \rho \theta_{*} - \phi_{*}  , a_* - a } \leq 4 \varepsilon_{\ell} = 2 \varepsilon_{\ell+1}.
$$
Therefore, the true MV gap incurred by a suboptimal action in $\mathcal{A}_{\ell}$ is at most $2 \varepsilon_\ell$.
% is at most $T_{\ell} \cdot 2 \varepsilon_{\ell}$. 
In other words, when $G$ happens, a suboptimal action $a$ with gap $\Delta_a$ will be eliminated before phase $\ell_a = \min \{\ell \geq 1: 2 \varepsilon_\ell < \Delta_a  \} = \lceil \log_2(2 / \Delta_a ) \rceil$. This also indicates 
\begin{align}\label{eq:eps_delta}
\varepsilon_{\ell_a}\geq\frac{\Delta_a}{4}\,.
\end{align}

By setting $\delta = {1}/{ T}$, we can therefore bound the quantity $\E{\tau_a(T)} $:
\begin{eqnarray}
\E{\tau_a(T)} &\leq&  \frac{1}{T} \cdot T  + (1-\frac{1}{T}) \sum_{\ell=1}^{\ell_a} n_{\ell,a} \nonumber \\ 
&\leq& 1 + \sum_{\ell=1}^{\ell_a} \left\lceil \hat{C}^2 \frac{d^{2} g_{\ell}(Q_{\ell}^{*}) \log(d) Q_{\ell}^{*} (a) }{\varepsilon_{\ell}^{2}} \log^2 \left(\frac{ K T }{\delta}\right)\right\rceil \\
&\leq& 1 + \sum_{\ell=1}^{\ell_a} \left( \hat{C}^2 \frac{d^{3}  \log(d) Q^{*}_{\ell} (a)}{\varepsilon_{\ell}^{2}} \log^{2} \left(\frac{ K T^{} }{\delta}\right) + 1 \right)  \nonumber \\
&\leq& 1 +  \hat{C}^{2} d^{3} \log(d) \log^2(K T^{2}) \sum_{\ell=1}^{\ell_a}  \frac{Q^*_{l}(a)}{\varepsilon_\ell^{2}}  + \ell_a  \nonumber\\ 
&\leq& 1 +  \hat{C}^{2} d^{3} \log(d) \log^2(K T^{2})  \frac{\sum_{\ell=1}^{\ell_a}  Q^*_{l}(a)}{\varepsilon_{\ell_a}^{2}}  + \log \left( \frac{2}{\Delta_a} \right) + 1  \nonumber \\
&\leq& 2 +  \frac{16\hat{C}^{2} d^{3} \log(d) \log^2(K T^{2})}{\Delta^2_a}  \left(\sum_{\ell=1}^{\ell_a}  Q^*_{l}(a)\right)  +  \log \left( \frac{2}{\Delta_a} \right) \,.  \nonumber 
%&=& O\left(  \frac{d^{3} \log(d)   \log^2(K T) } {\Delta_a^2 }  + \log({\Delta_a}^{-1}) \right) .
\end{eqnarray}
Here, the second last inequality uses the fact that $\epsilon_{l-1}>\epsilon_l$ and the last step uses \eqref{eq:eps_delta}.
Therefore, noting the simple algebraic fact that $\log \left( 2 / \Delta \right) <  1/\Delta^2$ for positive $\Delta$, we conclude that 
$$
\E{\tau_a(T)} \leq  O \left(  \frac{ d^{3} \log(d) \log^2(K T)}{\Delta^2_a}  \left( \sum_{\ell=1}^{\ell_a}  Q^*_{l}(a) \right)   \right) . 
$$
\fi 





% \Jingwei{In the last two lines, $\log({\Delta_a}^{-1})$ should be $\lceil \log_2(2 / \Delta_a ) \rceil$? Shall we also include this term in Eq. 28?   }
% \Ruihao{Oh yes, please change them to $\lceil \log_2(2 / \Delta_a ) \rceil$ if needed. We do not need to include this, it appears to me that $\log(\Delta^{-1})$ is dominated by $1/\Delta^2$?}
% \Jingwei{Yes. $\log \left( \frac{2}{\Delta} \right) <  1/\Delta^2$ for positive $\Delta$. I checked using $Plot[Log[2/x] - 1/x^2, {x, 0, 100}]$ in Mathematica. But I have a very basic question of whether we should report$ \E{\tau_a(T)} \leq  O \left(  \frac{ d^{3} \log(d) \log^2(K T^{2})}{\Delta^2_a}  \left( \sum_{\ell=1}^{\ell_a}  Q^*_{l}(a) \right)    \right) $ or $ \E{\tau_a(T)} \leq  O \left(  \frac{ d^{3} \log(d) \log^2(K T^{2})}{\Delta^2_a}  \left( \sum_{\ell=1}^{\ell_a}  Q^*_{l}(a) \right)   + \log \left( \frac{1}{\Delta_a} \right) \right) $. Because we have to sum over $K$, if we do the latter, we will have a $\sum_{a \in \mathcal{A}} \log( 1 / \Delta_a )$ in the bound on the regret, which is linear in $K$. If we do the former, the $K$ dependence on the proxy regret would be only of $\log(K)$. Now I kept the latter one. } \Ruihao{You would only have this term for those who has $Q^*_l(a)\geq 0\,.$ So remove this.}
\iffalse


\begin{equation} \label{eq:phase_elimination_phase_length}
    n_{\ell,a}=\left\lceil \hat{C}^2 \frac{d^{2} g_{\ell}(Q_{\ell}^{*}) \log(d) Q_{\ell}^{*} (a) }{\varepsilon_{\ell}^{2}} \log^2 \left(\frac{ K T }{\delta}\right)\right\rceil 
\end{equation}

By setting $\delta = \frac{1}{ T}$, we can therefore bound the quantity $\E{\tau_a(T)} $:
\begin{eqnarray}
\E{\tau_a(T)} &\leq&  \frac{1}{T} \cdot T  + (1-\frac{1}{T}) \sum_{\ell=1}^{\ell_a} n_{\ell,a} \nonumber \\ 
&\leq& 1 + \sum_{\ell=1}^{\ell_a} n_{(\ell)} \\
&\leq& 1 + \sum_{\ell=1}^{\ell_a} \left( \hat{C}^2 \frac{d^{3}  \log(d) Q^{*}_{\ell} (a)}{\varepsilon_{\ell}^{2}} \log^{2} \left(\frac{ K T^{} }{\delta}\right) + \frac{d(d+1)}{2} \right)  \nonumber \\
&=& 1 +  \hat{C}^{2} d^{3} \log(d) \log^2(K T^{2}) \sum_{\ell=1}^{\ell_a}  \frac{1}{\varepsilon_\ell^{2}}  + \ell_a \cdot \frac{d(d+1)}{2} \nonumber \\
&=& O\left(  \frac{d^{3} \log(d)   \log^2(K T^2) } {\Delta_a^2 }  + d^2\log(\frac{1}{\Delta_a}) \right) .
\end{eqnarray}

\fi 

